Gaia Data Release 3: Microlensing Events from All Over the Sky

Context: One of the rarest types of variability is the phenomenon of gravitational microlensing, a transient brightening of a background star due to an intervening lensing object. Microlensing is a powerful tool in studying the invisible or otherwise undetectable populations in the Milky Way, including planets and black holes. Aims: We describe the first Gaia catalogue of microlensing event candidates, give an overview of its content and discuss its validation. Methods: The catalogue of Gaia microlensing events is composed by analysing the light curves of around 2 billion sources of Gaia Data Release 3 from all over the sky covering 34 months between 2014 and 2017. Results: We present 363 Gaia microlensing events and discuss their properties. Ninety events were never reported before and were not discovered by other surveys. The contamination of the catalogue is assessed to 0.6-1.7%.

==> GDR3_master_include.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% !!! DO NOT MODIFY THIS FILE !!! %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% !!! DO NOT MODIFY THIS FILE !!! %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% !!! DO NOT MODIFY THIS FILE !!! %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% !!! DO NOT MODIFY THIS FILE !!! %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% !!! DO NOT MODIFY THIS FILE !!! %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% !!! DO NOT MODIFY THIS FILE !!! %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% !!! DO NOT MODIFY THIS FILE !!! %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% !!! DO NOT MODIFY THIS FILE !!! %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% !!! DO NOT MODIFY THIS FILE !!! %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% !!! DO NOT MODIFY THIS FILE !!! %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{natbib}
\usepackage{graphicx,epstopdf}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{url}
%\usepackage{mathptmx}
\usepackage{alltt}
\usepackage{listings}
\usepackage{lineno}
\usepackage{txfonts}
\RequirePackage{array}
\usepackage{makeidx}
\usepackage{multirow}
\usepackage{xspace}
\usepackage{longtable}
\usepackage[utf8]{inputenc}
\usepackage{float}
\usepackage{nameref}
\usepackage{color}
\usepackage{hyperref}

\newcommand*\aatablefootname{Notes}
\newcommand*\aatablefootfont{\small}
\newcommand*\aatablefootnamefont{\small\bfseries}
\newlength{\VSpaceBeforeTabBib}
\setlength{\VSpaceBeforeTabBib}{2ex}
\newlength{\VSpaceBeforeTabFoot}
\setlength{\VSpaceBeforeTabFoot}{2ex}

\newcommand\tablefoot[1]{\VSpaceBeforeTabBib=1ex%
\par\vspace{\VSpaceBeforeTabFoot}
\noindent
\begin{minipage}{\linewidth}
{\aatablefootnamefont\aatablefootname.}~%
\aatablefootfont
\ignorespaces
#1%
\end{minipage}%
}
\newcommand*\tablefootmark[1]{%
\unskip
\hbox{\@textsuperscript{\normalfont\itshape\ignorespaces#1}}%
\,%
\ignorespaces
}
\newcommand\tablefoottext[2]{%
\hbox{\@textsuperscript{\normalfont({\itshape\ignorespaces#1})}}%
~%
\ignorespaces
#2\ \ignorespaces%
}


\DeclareRobustCommand{\object}[1]{%
   #1%
   \addcontentsline{obj}{obj}{#1}%
}

% Macro for rendering vectors 
% Added to display matrices correctly
%\renewcommand{\vec}[1]{\ensuremath{\mathchoice{\mbox{\boldmath$\displaystyle#1$}}
%{\mbox{\boldmath$\textstyle#1$}}
%{\mbox{\boldmath$\scriptstyle#1$}}
%{\mbox{\boldmath$\scriptscriptstyle#1$}}}}

%\def\vec#1{\ensuremath{\mathbf{#1}}}
\renewcommand*\vec[1]{\ensuremath{\boldsymbol{#1}}}

% Macro for rendering tensors
\newcommand*\tens[1]{\ensuremath{\mathsf{#1}}}

% Macro for rendering quaternions in math mode
\newcommand{\quat}[1]{\mathbf{#1}}

\def\arxivprefixe{arXiv}
\def\arxivprefixesep{:}
\def\arxiv#1{%
{\tt \arxivprefixe\arxivprefixesep\ignorespaces#1}%
}
\newcommand{\eprint}[2][]{%
{\tt\if!#1!#2\else#1\arxivprefixesep\ignorespaces#2\fi}%
}

\bibpunct{(}{)}{;}{a}{}{,}

% Macros for referencing
\providecommand{\charef}[1]{Chapter~\ref{#1}}
\providecommand{\secref}[1]{Section~\ref{#1}}
\providecommand{\tabref}[1]{Table~\ref{#1}}
\providecommand{\figref}[1]{Figure~\ref{#1}}
\providecommand{\equref}[1]{Equation~\ref{#1}}

\renewcommand{\glossary}[1]{#1}

% For use outside of Maths mode
% \def\deg{\,$^\circ$}
% \def\arcmin{\,$'$}
% \def\arcsec{\,$''$}
%\def\deg{\hbox{$^\circ$}}
%\def\arcmin{\hbox{$'$}}
%\def\arcsec{\hbox{$''$}}
%\def\fd{\hbox{$.\!\!^{\rm d}$}}
%\def\fh{\hbox{$.\!\!^{\rm h}$}}
%\def\fm{\hbox{$.\!\!^{\rm m}$}}
%\def\fs{\hbox{$.\!\!^{\rm s}$}}
%\def\fdg{\hbox{$.\!\!^\circ$}}
%\def\farcm{\hbox{$.\mkern-4mu^\prime$}}
%\def\farcs{\hbox{$.\!\!^{\prime\prime}$}}

% Redefined without \hbox; for use in math and text mode

\def\deg{\ensuremath{^\circ}}
\def\arcmin{\ensuremath{'}}
\def\arcsec{\ensuremath{''}}
\def\fd{\ensuremath{.\!\!^{\mathrm d}}}
\def\fh{\ensuremath{.\!\!^{\mathrm h}}}
\def\fm{\ensuremath{.\!\!^{\mathrm m}}}
\def\fs{\ensuremath{.\!\!^{\mathrm s}}}
\def\fdg{\ensuremath{.\!\!^\circ}}
\def\farcm{\ensuremath{.\mkern-4mu^\prime}}
\def\farcs{\ensuremath{.\!\!^{\prime\prime}}}

%\providecommand{\secs}{\,s}
%\providecommand{\ms}{\,m\,s$^{-1}$}
%\providecommand{\kms}{\,km\,s$^{-1}$}
%\providecommand{\masyr}{\,mas\,yr$^{-1}$}
%\providecommand{\muas}{\,$\mu$as}
%\providecommand{\muasyr}{\muas\,yr$^{-1}$}

% redefined for use in math and text mode
\providecommand{\secs}{\ensuremath{\,\rm s}\xspace}
\providecommand{\ms}{\ensuremath{\rm \,m\,s^{-1}}\xspace}
\providecommand{\kms}{\ensuremath{\rm \,km\,s^{-1}}\xspace}
\providecommand{\masyr}{\ensuremath{\rm \,mas\,yr^{-1}}\xspace}
\providecommand{\massec}{\ensuremath{\rm \,mas\,s^{-1}}\xspace}
\providecommand{\muas}{\ensuremath{\,\mu\textnormal{as}}\xspace}
\providecommand{\muasyr}{\ensuremath{\muas\,\rm yr^{-1}}\xspace}
% requested by CU4 in November 2021
\providecommand{\massec}{\ensuremath{\rm \,mas\,s^{-1}}\xspace}

% Computing terms
\providecommand{\inp}[1]{{\tt #1}}
\providecommand{\prog}[1]{{\it #1}}
\providecommand{\class}[1]{{\it #1}}
\providecommand{\pack}[1]{{\em #1}}
\providecommand{\property}[1]{{\em #1}}
\providecommand{\method}[1]{{\em #1}}
\providecommand{\file}[1]{{\em #1}}
\providecommand{\directory}[1]{{\em #1}}
\providecommand{\code}[1]{{\tt #1}}

% Data Model terms
\providecommand{\dt}[1]{{\tt #1}}
% Common variable star types
\newcommand{\rrl}{RR~Lyrae\xspace}
\newcommand{\rrab}{RRab\xspace}
\newcommand{\rrc}{RRc\xspace}
\newcommand{\rrd}{RRd\xspace}
\newcommand{\ttwocep}{Type~II Cepheid\xspace}
\newcommand{\dscuti}{$\delta$~Scuti\xspace}
\newcommand{\bcep}{$\beta$~Cephei\xspace}
\newcommand{\zzceti}{ZZ~Ceti\xspace}
\newcommand{\amcvn}{AM~CVn\xspace}
\newcommand{\roap}{roAp\xspace}
\newcommand{\dcep}{$\delta$~Cepheid\xspace}
\newcommand{\rvtauri}{RV~Tauri\xspace}
\newcommand{\wvirg}{W~Virginis\xspace}
\newcommand{\blherc}{BL~Herculis\xspace}
\newcommand{\acep}{ACEP\xspace}
\newcommand{\cep}{Cepheid\xspace}
\newcommand{\ulens}{Microlensing\xspace}

%Related to CU7 processing and analysis
\newcommand\geqfov[1]{$\geq$#1~FoV\xspace}
\newcommand{\rtwoone}{$R_{21}$\xspace}
\newcommand{\phitwoone}{$\phi_{21}$\xspace}
\newcommand{\pvalue}{$p$-value\xspace}
\newcommand{\rthreeone}{$R_{31}$\xspace}
\newcommand{\phithreeone}{$\phi_{31}$\xspace}

%Related to CU6 processing and analysis

%\newcommand{\RV}{$\varv_{\rm rad}$ }
%\newcommand{\RV}{$V_{\rm rad}$\xspace}
% redefined for use in text and math mode
\newcommand{\RV}{\ensuremath{V_{\rm rad}}\xspace}
%Related to CU8 processing and analysis

\providecommand{\maspyr}{\muasyr}
\providecommand{\deriv}{\ensuremath{\mathrm{d}}}
\providecommand{\given}{\ensuremath{\hspace{0.1em}\mid\hspace{0.1em}}}

%\providecommand{\um}{\,$\mu$m}
%\providecommand{\erg}{\,erg}
%\providecommand{\ergs}{\,erg~s}
%\providecommand{\yr}{\,yr}
%\providecommand{\Myr}{\,Myr}
%\providecommand{\Gyr}{\,Gyr}
%\providecommand{\pc}{\,pc}
%\providecommand{\kpc}{\,kpc}
%\providecommand{\Mpc}{\,Mpc}
%\providecommand{\Lsun}{\,${\cal L}_{\odot}$}
%\providecommand{\Msun}{\,${\cal M}_{\odot}$}
%\providecommand{\Rsun}{\,${\cal R}_{\odot}$}
%\providecommand{\Zsun}{\,${\cal Z}_{\odot}$}
%\providecommand{\ang}{\,$\text{\AA}$}
%\providecommand{\mas}{\,mas}
%\providecommand{\sigparallax}{\ensuremath{\sigma_{\varpi}}}
%\providecommand{\dist}{\ensuremath{r}}
%\providecommand{\dist}{\,$r$} % distance to source from Sun
%\providecommand{\aabun}{\ensuremath{[\alpha/\mathrm{H}]}}
%\providecommand{\lum}{\ensuremath{{\cal L}}}
%\providecommand{\mass}{\ensuremath{{\cal M}}}
%\providecommand{\radius}{\ensuremath{{\cal R}}}
%\providecommand{\Zabun}{\ensuremath{{\cal Z}}}
%\providecommand{\ebpminrp}{\ensuremath{E(G_{\rm BP} - G_{\rm RP})}}
%\providecommand{\ebpminrp}{\ensuremath{E({\rm BP} - {\rm RP})}}
\providecommand{\bcg}{\ensuremath{\mathrm{BC}_G}\xspace}
%\providecommand{\mbolsun}{$M_{\rm bol}$}
%\providecommand{\Tsun}{\ensuremath{{T_{{\rm eff}{\odot}}}}}
% software names for consistency
%\def\gspphot{GSP-Phot\xspace}
%\def\priam{Priam\xspace}
%\def\flame{FLAME\xspace}
%\def\apsis{Apsis\xspace}
\def\extratrees{\textsc{ExtraTrees}\xspace}

% Related to CU8 processing and analysis redefined for use in text and math mode, xspace added
\providecommand {\um}{\ensuremath{\,\mu\mathrm{m}}\xspace}
\providecommand{\erg}{\ensuremath{\,\rm erg}\xspace}
\providecommand{\ergs}{\ensuremath{\,\rm erg~s}\xspace}
\providecommand{\yr}{\ensuremath{\,\rm yr}\xspace}
\providecommand{\Myr}{\ensuremath{\,\rm Myr}\xspace}
\providecommand{\Gyr}{\ensuremath{\,\rm Gyr}\xspace}
\providecommand{\pc}{\ensuremath{\,\rm pc}\xspace}
\providecommand{\kpc}{\ensuremath{\,\rm kpc}\xspace}
\providecommand{\Mpc}{\ensuremath{\,\rm Mpc}\xspace}
\providecommand{\Lsun}{\ensuremath{\,{\cal L}_{\odot}}\xspace}
\providecommand{\Msun}{\ensuremath{\,{\cal M}_{\odot}}\xspace}
\providecommand{\Rsun}{\ensuremath{\,{\cal R}_{\odot}}\xspace}
\providecommand{\Zsun}{\ensuremath{\,{\cal Z}_{\odot}}\xspace}
\providecommand{\ang}{\ensuremath{\text{\,\AA}}\xspace}
\providecommand{\mas}{\ensuremath{\,\mathrm{mas}}\xspace}
\providecommand{\sigparallax}{\ensuremath{\sigma_{\varpi}}\xspace}
\providecommand{\dist}{\ensuremath{\,r}\xspace} % distance to source from Sun
\providecommand{\aabun}{\ensuremath{[\alpha/\mathrm{H}]}\xspace}
\providecommand{\lum}{\ensuremath{{\cal L}}\xspace}
\providecommand{\mass}{\ensuremath{{\cal M}}\xspace}
\providecommand{\radius}{\ensuremath{{\cal R}}\xspace}
\providecommand{\Zabun}{\ensuremath{{\cal Z}}\xspace}
\newcommand{\bpminrp}{\ensuremath{G_\mathrm{BP}-G_\mathrm{RP}}\xspace}
\providecommand{\ebpminrp}{\ensuremath{E(G_{\rm BP} - G_{\rm RP})}\xspace}
\providecommand{\mbolsun}{\ensuremath{M_{\rm bol}}\xspace}
\providecommand{\Tsun}{\ensuremath{{T_{{\rm eff}{\odot}}}}\xspace}

% CU8 macros requested on 24 August 2021
\providecommand{\prob}[2]{\ensuremath{{P^#1_#2}}}
\providecommand{\prior}[2]{\ensuremath{{\pi^#1_#2}}}

%CU8 macros requested on 30 October 2021
\newcommand{\matfont}[1]{\ensuremath{\boldsymbol{\mathsf{#1}}}}
%\newcommand{\mat}[1]{\matfont{#1}}
\newcommand{\mat}[1]{\vec{#1}}
\newcommand{\ion}[2]{#1\,\textsc{\lowercase{#2}}}

%CU8 module name macros
\providecommand{\modulename}[1]{#1\xspace}
\providecommand{\apsis}{\modulename{Apsis}}
\providecommand{\smsgen}{\modulename{SMSgen}}
\providecommand{\dsc}{\modulename{DSC}}
\providecommand{\gspphot}{\modulename{GSP-Phot}}
\providecommand{\priam}{\modulename{Priam}}
\providecommand{\aeneas}{\modulename{Aeneas}}
\providecommand{\gspspec}{\modulename{GSP-Spec}}
\providecommand{\msc}{\modulename{MSC}}
\providecommand{\flame}{\modulename{FLAME}}
\providecommand{\espels}{\modulename{ESP-ELS}}
\providecommand{\esphs}{\modulename{ESP-HS}}
\providecommand{\espcs}{\modulename{ESP-CS}}
\providecommand{\espucd}{\modulename{ESP-UCD}}
\providecommand{\ugc}{\modulename{UGC}}
\providecommand{\oa}{\modulename{OA}}
\providecommand{\oca}{\modulename{OCA}}
\providecommand{\qsoc}{\modulename{QSOC}}
\providecommand{\tge}{\modulename{TGE}}

% Macro for rendering authors' names
\providecommand{\authors}[1]{\nobreak\textbf{Author(s): \author{#1}}\par}

% Macro for rendering references to large versions of images
% Use this version for tests and HTML
\providecommand{\viewLarge}[1]{\href{/archive/documentation/GDR3/large/#1}{(large image)}}

% Macros for rendering Gaia terms and related satellite projects' names
%\newcommand\gaia{Gaia}
%\newcommand\hip{Hipparcos}
%\newcommand\tyc{Tycho}
%\newcommand\bpminrp{\ensuremath{G_\mathrm{BP}-G_\mathrm{RP}}}
%\newcommand\tyctwo{Tycho-2}
\newcommand\gdr[1]{\gaia~DR#1}
%macro for rendering Gaia Early Data Release names
\newcommand\egdr[1]{\gaia~EDR#1}

\newcommand{\gaia}{Gaia\xspace}
\newcommand{\hip}{Hipparcos\xspace}
\newcommand{\tyc}{Tycho\xspace}
\newcommand{\bporrp}{BP/RP\xspace}
\newcommand{\tyctwo}{Tycho-2\xspace}

%my revised definition
%\newcommand{\gdr}[2][]{\gaia~#1DR#2}

%Jos' definition
%\makeatletter
%\def\gdr{@ifnextchar[{@with}{@without}}
%\def@with1#2{\gaia~#1DR#2}
%\def@without#1{\gaia~DR#1}
%\makeatother


%\makeatletter
%\newcommand{\gdr}{\@ifnextchar[{\@gdr}{\@gdr[]}}
%\def\@gdr[#1]#2{\gaia~#1DR#2}
%\makeatother

%\def\mmag{mmag\xspace}
%\def\parallax{$\varpi$}
\def\teff{\ensuremath{T_{\rm eff}}\xspace}
\def\logg{\ensuremath{\log g}\xspace}
%\def\feh{[Fe/H]\xspace}
%\def\mh{[M/H]\xspace}
%\def\a0{\ensuremath{A_{\rm 0}}}
%\def\ag{\ensuremath{A_{\rm G}}}
%\def\abp{\ensuremath{A_{\rm BP}}}
%\def\arp{\ensuremath{A_{\rm RP}}}
%\def\av{$A_{\rm V}$}
%\def\atge{$A_{\rm TGE}$}
%\def\relext{$R_{\rm 0}$}
%\def\mg{$M_{\rm G}$}
% \def\aabun{[$\alpha$/Fe]}
%\def\vsini{$v\sin i$}
\def\gmag{\ensuremath{G}\xspace}
\def\gbp{\ensuremath{G_{\rm BP}}\xspace}
\def\grp{\ensuremath{G_{\rm RP}}\xspace}
\def\grvs{\ensuremath{G_{\rm RVS}}\xspace}
\def\gminr{\ensuremath{G-G_{\rm RP}}\xspace}
\def\bming{\ensuremath{G_{\rm BP}-G}\xspace}
%\def\cat{\ion{Ca}{ii}}

% redefined for use in text and math mode and/or xspace added
\def\mmag{\ensuremath{\,\rm mmag}\xspace}
\def\parallax{\ensuremath{\varpi}\xspace}
\def\feh{\ensuremath{[\rm Fe/H]}\xspace}
\def\mh{\ensuremath{[\rm M/H]}\xspace}
\def\a0{\ensuremath{A_{\rm 0}}\xspace}
\def\ag{\ensuremath{A_{\rm G}}\xspace}
\def\abp{\ensuremath{A_{\rm BP}}\xspace}
\def\arp{\ensuremath{A_{\rm RP}}\xspace}
\def\av{\ensuremath{A_{\rm V}}\xspace}
\def\atge{\ensuremath{A_{\rm TGE}}\xspace}
\def\relext{\ensuremath{R_{\rm 0}}\xspace}
\def\mg{\ensuremath{M_{\rm G}}\xspace}
\def\vsini{\ensuremath{v\sin i}\xspace}
%
% Bibliography and bibfile
\def\aj{AJ}%
          % Astronomical Journal
\def\actaa{Acta Astron.}%
          % Acta Astronomica
\def\araa{ARA\&A}%
          % Annual Review of Astron and Astrophys
\def\apj{ApJ}%
          % Astrophysical Journal
\def\apjl{ApJ}%
          % Astrophysical Journal, Letters
\def\apjs{ApJS}%
          % Astrophysical Journal, Supplement
\def\ao{Appl.~Opt.}%
          % Applied Optics
\def\apss{Ap\&SS}%
          % Astrophysics and Space Science
\def\aap{A\&A}%
          % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}%
          % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}%
          % Astronomy and Astrophysics, Supplement
\def\azh{AZh}%
          % Astronomicheskii Zhurnal
\def\baas{BAAS}%
          % Bulletin of the AAS
\def\bac{Bull. astr. Inst. Czechosl.}%
          % Bulletin of the Astronomical Institutes of Czechoslovakia 
\def\caa{Chinese Astron. Astrophys.}%
          % Chinese Astronomy and Astrophysics
\def\cjaa{Chinese J. Astron. Astrophys.}%
          % Chinese Journal of Astronomy and Astrophysics
\def\icarus{Icarus}%
          % Icarus
\def\jcap{J. Cosmology Astropart. Phys.}%
          % Journal of Cosmology and Astroparticle Physics
\def\jrasc{JRASC}%
          % Journal of the RAS of Canada
\def\mnras{MNRAS}%
          % Monthly Notices of the RAS
\def\memras{MmRAS}%
          % Memoirs of the RAS
\def\na{New A}%
          % New Astronomy
\def\nar{New A Rev.}%
          % New Astronomy Review
\def\pasa{PASA}%
          % Publications of the Astron. Soc. of Australia
\def\pra{Phys.~Rev.~A}%
          % Physical Review A: General Physics
\def\prb{Phys.~Rev.~B}%
          % Physical Review B: Solid State
\def\prc{Phys.~Rev.~C}%
          % Physical Review C
\def\prd{Phys.~Rev.~D}%
          % Physical Review D
\def\pre{Phys.~Rev.~E}%
          % Physical Review E
\def\prl{Phys.~Rev.~Lett.}%
          % Physical Review Letters
\def\pasp{PASP}%
          % Publications of the ASP
\def\pasj{PASJ}%
          % Publications of the ASJ
\def\qjras{QJRAS}%
          % Quarterly Journal of the RAS
\def\rmxaa{Rev. Mexicana Astron. Astrofis.}%
          % Revista Mexicana de Astronomia y Astrofisica
\def\skytel{S\&T}%
          % Sky and Telescope
\def\solphys{Sol.~Phys.}%
          % Solar Physics
\def\sovast{Soviet~Ast.}%
          % Soviet Astronomy
\def\ssr{Space~Sci.~Rev.}%
          % Space Science Reviews
\def\zap{ZAp}%
          % Zeitschrift fuer Astrophysik
\def\nat{Nature}%
          % Nature
\def\iaucirc{IAU~Circ.}%
          % IAU Cirulars
\def\aplett{Astrophys.~Lett.}%
          % Astrophysics Letters
\def\apspr{Astrophys.~Space~Phys.~Res.}%
          % Astrophysics Space Physics Research
\def\bain{Bull.~Astron.~Inst.~Netherlands}%
          % Bulletin Astronomical Institute of the Netherlands
\def\fcp{Fund.~Cosmic~Phys.}%
          % Fundamental Cosmic Physics
\def\gca{Geochim.~Cosmochim.~Acta}%
          % Geochimica Cosmochimica Acta
\def\grl{Geophys.~Res.~Lett.}%
          % Geophysics Research Letters
\def\jcp{J.~Chem.~Phys.}%
          % Journal of Chemical Physics
\def\jgr{J.~Geophys.~Res.}%
          % Journal of Geophysics Research
\def\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\def\memsai{Mem.~Soc.~Astron.~Italiana}%
          % Mem. Societa Astronomica Italiana
\def\nphysa{Nucl.~Phys.~A}%
          % Nuclear Physics A
\def\physrep{Phys.~Rep.}%
          % Physics Reports
\def\physscr{Phys.~Scr}%
          % Physica Scripta
\def\planss{Planet.~Space~Sci.}%
          % Planetary Space Science
\def\procspie{Proc.~SPIE}%
          % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

\def\ltsim{\ifmmode\stackrel{<}{_{\sim}}\else$\stackrel{<}{_{\sim}}$\fi}
\hyphenation{mag-ni-tude}
%
% Page layout
%

\setlength{\textwidth}{16cm}
\setlength{\textheight}{22cm}

\setlength{\topmargin}{0cm}
\setlength{\oddsidemargin}{0cm}
\setlength{\evensidemargin}{0cm}
\setlength{\leftmargini}{2cm}
\setlength{\marginparwidth}{2cm}

\setlength{\parindent}{0in}             % No indent at start of paragraphs
\setlength{\parskip}{\baselineskip}     % Blank line between paragraph
%\setlength\headheight{35pt}            % Make space for logo

% added to control formatting of TOC, LOT and LOF entries
\renewcommand{\numberline}[1]{#1~}

\setcounter{secnumdepth}{6}

\hypersetup{baseurl=https://gea.esac.esa.int}

% macro for controlling vertical alignment of numbers in table columns, requested by CU4
\newcommand{\digs}[1]{\count0=#1 \loop \ifnum\count0>0 \advance\count0 by -1 \phantom{0}\repeat}

% Macro for writing of Data Model table field names that contain underscores.
%original definition
%\begingroup\@fieldName\scantokens{\tt\small #1\endinput}\endgroup}
% another non-working version 
%\begingroup\@fieldName\scantokens{{\tt{\small #1}}\endinput}\endgroup}
%\makeatletter
%\DeclareRobustCommand*{\fieldName}[1]{%
%  \begingroup\@fieldName\scantokens{\tt\small #1}\endgroup}
%\begingroup\lccode`\~=`\_\relax
%   \lowercase{\endgroup\def\@fieldName{\catcode`\_=\active \let~\_}}
%\makeatother
 
\makeatletter
\DeclareRobustCommand*{\fieldName}[1]{%
  \begingroup\@fieldName\scantokens{\texttt{\small {#1}}\noexpand}\endgroup}
\begingroup\lccode`\~=`\_\relax
   \lowercase{\endgroup\def\@fieldName{\catcode`\_=\active \let~\_}}
\makeatother

==> table-events-uniq-sort-mag-j2000-trim.tex <==
001 & 6059400613544951552 & 184.4363263 & -59.0294197 & 298.6005085 & 3.5586850 & 13.58 & A \\ 
002 & 4135677580466393216 & 258.0716963 & -16.8677137 & 6.0098740 & 12.9894820 & 13.64 & A \\ 
003 & 4084984459435880064 & 284.4366819 & -20.7757293 & 14.9165537 & -10.6404670 & 14.16 & A \\ 
004 & 4043236380953360512 & 268.4052228 & -33.1237924 & 357.2830138 & -3.6192437 & 14.38 & A \\ 
005 & 4046189531753775872 & 276.2347519 & -30.9712872 & 2.3615295 & -8.4309626 & 14.40 & A \\ 
006 & 5369575367669793536 & 175.9545194 & -51.7786254 & 292.4152033 & 9.7070281 & 14.74 & A \\ 
007 & 4042926314286962944 & 270.2539729 & -32.6895521 & 358.4346692 & -4.7498989 & 14.78 & A \\ 
008 & 6028496189222706432 & 255.7845506 & -31.2111200 & 352.9458509 & 6.3248291 & 15.00 & A \\ 
009 & 4103350800428736384 & 279.8111863 & -15.4369500 & 17.8014157 & -4.3444691 & 15.08 & A \\ 
010 & 4056251952898990848 & 269.5945985 & -29.9489827 & 0.5437424 & -2.9060128 & 15.16 & A \\ 
011 & 4093461453632265600 & 279.0502629 & -18.0503157 & 15.1331452 & -4.8801400 & 15.23 & A+B \\ 
012 & 5305778988625143296 & 143.5517537 & -57.8164443 & 279.0375096 & -4.4075008 & 15.46 & A \\ 
013 & 4052272339270449024 & 274.7611076 & -27.7293739 & 4.6769250 & -5.8077405 & 15.53 & A \\ 
014 & 4050176120351393792 & 270.6320911 & -30.1235644 & 0.8360192 & -3.7732156 & 15.61 & B \\ 
015 & 4053164279372999680 & 276.0098469 & -25.1043278 & 7.5357066 & -5.5861482 & 15.67 & A \\ 
016 & 5882824406244672256 & 234.7379625 & -56.0303213 & 324.8332656 & -0.4528306 & 15.96 & A \\ 
017 & 4041047008398705664 & 267.0329353 & -35.5803325 & 354.5860534 & -3.8936482 & 15.97 & A \\ 
018 & 4050208551598764032 & 271.1193843 & -29.8161981 & 1.3115071 & -3.9914357 & 16.00 & A+B \\ 
019 & 4159994512750671232 & 275.9289525 & -7.3020659 & 23.2666791 & 2.7836325 & 16.01 & A \\ 
020 & 4067907184112930944 & 265.7034019 & -25.5169917 & 2.5881853 & 2.3205060 & 16.03 & A \\ 
021 & 4041238259061973504 & 264.6744198 & -35.5066956 & 353.6436127 & -2.2195980 & 16.06 & A \\ 
022 & 5956630082001769984 & 269.5337814 & -42.5974274 & 349.4320429 & -9.0692191 & 16.08 & A \\ 
023 & 6059816980526317568 & 191.5840141 & -58.8941185 & 302.2714390 & 3.9710873 & 16.11 & B \\ 
024 & 5951752068649725312 & 262.4024369 & -46.2347526 & 343.6506395 & -6.5542396 & 16.13 & A \\ 
025 & 4108020361965432064 & 260.8780868 & -27.3787487 & 358.6732768 & 4.9403756 & 16.14 & A+B \\ 
026 & 5515709499618656768 & 127.4644053 & -47.1922367 & 264.6184588 & -4.7449336 & 16.17 & A \\ 
027 & 4039110875886635008 & 271.1335543 & -34.8929303 & 356.8557550 & -6.4587185 & 16.25 & A \\ 
028 & 4041760939405737344 & 266.8708058 & -34.1758834 & 355.7240287 & -3.0570121 & 16.29 & A \\ 
029 & 4063277591626468608 & 271.8813320 & -26.6791216 & 4.3856614 & -3.0549313 & 16.32 & B \\ 
030 & 4050909181279109888 & 273.1546856 & -27.8870166 & 3.8672279 & -4.6272229 & 16.33 & B \\ 
031 & 4062254461725875328 & 270.0523139 & -29.7174753 & 0.9422900 & -3.1359064 & 16.33 & B \\ 
... &             ...                            & ...                  & ...                   & ...               & ...                & ...       & ...\\

==> table-sort-id-xm-trim.tex <==
007 & OGLE-2015-BLG-0064\\
008 & BLG896.14.123\\
010 & OGLE-2016-BLG-0133 KMT-2016-BLG-0485\\
011 & BLG586.01.37855\\
013 & OGLE-2015-BLG-1755\\
014 & BLG513.13.37217 OGLE-2015-BLG-0056\\
018 & BLG513.19.77649 OGLE-2016-BLG-1396 KMT-2016-BLG-0738\\
021 & OGLE-2016-BLG-0357\\
023 & GD2233.02.17021 ASASSN-16oe\\
025 & BLG921.22.94\\
026 & GD2110.04.10077\\
029 & BLG518.22.135316 OGLE-2015-BLG-1578 MOA-2015-BLG-338\\
030 & BLG523.06.68137 OGLE-2014-BLG-1948 MOA-2014-BLG-594\\
031 & BLG513.25.80350 OGLE-2016-BLG-1654 MOA-2016-BLG-457 KMT-2016-BLG-0698\\
.... & ....\\
